Learned Low Precision Graph Neural Networks

Deep Graph Neural Networks (GNNs) show promising performance on a range of graph tasks, yet at present are costly to run and lack many of the optimisations applied to DNNs. We show, for the first time, how to systematically quantise GNNs with minimal or no loss in performance using Network Architecture Search (NAS). We define the possible quantisation search space of GNNs. The proposed novel NAS mechanism, named Low Precision Graph NAS (LPGNAS), constrains both architecture and quantisation choices to be differentiable. LPGNAS learns the optimal architecture coupled with the best quantisation strategy for different components in the GNN automatically using back-propagation in a single search round. On eight different datasets, solving the task of classifying unseen nodes in a graph, LPGNAS generates quantised models with significant reductions in both model and buffer sizes but with similar accuracy to manually designed networks and other NAS results. In particular, on the Pubmed dataset, LPGNAS shows a better size-accuracy Pareto frontier compared to seven other manual and searched baselines, offering a 2.3 times reduction in model size but a 0.4% increase in accuracy when compared to the best NAS competitor. Finally, from our collected quantisation statistics on a wide range of datasets, we suggest a W4A8 (4-bit weights, 8-bit activations) quantisation strategy might be the bottleneck for naive GNN quantisations.

==> sections/abstract.tex <==
\begin{abstract}
  Deep Graph Neural Networks (GNNs) show promising performance on a range of graph tasks, yet at present are costly to run and lack many of the optimisations applied to DNNs.
  We show, for the first time, how to systematically
  quantise GNNs with minimal or no loss in performance
  using Network Architecture Search (NAS).
  We define the possible
  quantisation search space of GNNs.
  The proposed novel NAS mechanism,
  named Low Precision Graph NAS (LPGNAS),
  constrains both architecture and quantisation
  choices to be differentiable.
  LPGNAS learns the optimal
  architecture coupled with
  the best quantisation strategy
  for different components in the GNN automatically
  using back-propagation in a single search round.
  On eight different datasets,
  solving the task of classifying unseen nodes in a graph,
  LPGNAS generates quantised models with
  significant reductions in both model
  and buffer sizes but with similar accuracy
  to manually designed networks
  and other NAS results.
  In particular, on the Pubmed dataset,
  LPGNAS shows a better size-accuracy Pareto frontier
  compared to seven other manual and searched
  baselines, offering a $2.3 \times$ reduction in model size but a $0.4\%$ increase in accuracy when compared to the best NAS competitor.
\end{abstract}


==> sections/impact.tex <==
\section*{Potential Broader Impact}
Prior research on the carbon footprint of machine learning
suggests that neural networks have a potential to play an important role in carbon emissions \cite{henderson2020towards,strubell2019energy}.
In the meantime, various researchers have suggested the deployment of Graph Neural Networks at a system level in data centers to help analyse large-scale graph inputs \cite{hamilton2017inductive}.
This works shows an automatic method that reduces the total cost of running GNN inference.
The proposed method has the potential to significantly reduce the amount of carbon emitted by running GNN inference at scale.

In terms of hardware, the proposed method shows it is possible for GNNs to retain accuracy with low-precision parameters and activations. The reductions in bitwidths, model sizes and buffer sizes translate to decreases in computation complexity, storage requirements and peak on-chip memory usage. 
These reduced requirements benefit existing hardware platforms such as GPUs and CPUs, and the collected quantisation statistics also provide insights for ML accelerator designers that are interested in accelerating GNN inference.

==> tables/citation.tex <==
\begin{table}[h!]
\caption{
    Accuracy and size comparison on
    Cora, Pubmed and Citeseer with
    data splits same as \citet{yang2016revisiting}.
    Our results are averaged across 3 independent runs.
    The numbers in bold show best accuracies.
}
\label{tab:citation:original}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cc|cccccc}
\toprule
\multirow{2}*{Method}   & \multirow{2}*{Quan}    & \multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{CiteSeer} & \multicolumn{2}{c}{PubMed} \\
                        &        & Accuracy    & Size       & Accuracy    & Size           & Accuracy   & Size \\
\midrule
GAT                     & float  & $82.9 \pm 0.0 \%$  & $369.5$KB   & $72.7 \pm 0.0 \%$  & $950.3$KB     & $79.0 \pm 0.0 \%$  & $129.6$KB\\
GAT                     & w4a8   & $82.4 \pm 0.0 \%$  & $46.2$KB    & $66.7 \pm 0.0 \%$  & $118.8$KB     & $71.7 \pm 0.0 \%$  & $16.2$KB\\
JKNet                   & float  & $80.9 \pm 0.0 \%$  & $214.9$KB   & $70.0 \pm 0.0 \%$  & $505.2$KB     & $78.5 \pm 0.0 \%$  & $94.4$KB\\
JKNet                   & w6a8   & $80.9 \pm 0.0 \%$  & $40.3$KB    & $60.3 \pm 0.1 \%$  & $94.7$KB      & $76.6 \pm 0.1 \%$  & $17.7$KB\\
\midrule
GraphNAS                & float  & $84.2 \pm 1.0 \%$ & $752.4$KB   & $73.1 \pm 0.9 \%$  & $7688.6$KB     & $79.6 \pm 0.4 \%$ & $791.1$KB\\
AGNN$^*$                & float  & $83.6 \pm 0.3\%$  & $200.0$KB   & $73.8 \pm 0.7 \%$  & $2840.0$KB     & $79.7 \pm 0.4 \%$ & $280.0$KB\\
PDNAS                   & float  & $84.5 \pm 0.6 \%$ &$1534.9$KB   & $73.5 \pm 0.3 \%$  & $3824.9$KB     & $79.7 \pm 0.6 \%$ & $812.7$KB\\
% \midrule
% Ours & $\mathbf{84.5 \pm 0.6 \%}$ & $73.5 \pm 0.3 \%$ & $\mathbf{79.7 \pm 0.6 \%}$\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}



